DateLogicQA: Benchmarking Temporal Biases in Large Language Models

This paper introduces DateLogicQA, a benchmark with 190 questions covering diverse date formats, temporal contexts, and reasoning types. We propose the Semantic Integrity Metric to assess tokenization quality and analyse two biases: Representation-Level Bias, affecting embeddings, and Logical-Level Bias, influencing reasoning outputs. Our findings provide a comprehensive evaluation of LLMs' capabilities and limitations in temporal reasoning, highlighting key challenges in handling temporal data accurately.

==> figures_latex/contributions.tex <==
\begin{figure}[htp]
\includegraphics[width=0.8\columnwidth]{figures/contribution.pdf}
\centering
\caption{Contributions Chart}
\label{fig:contri}
\end{figure}

==> figures_latex/embedding.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth]{figures/Llama-3.2-3B-Instruct_embeddings.png}
\centering
\caption{Representation level Temporal Bias Analysis using LLama 3.2 3B }
\label{fig:embeddings}
\end{figure*}


% \begin{figure*}[h!]
%     \centering
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/Llama-3.2-3B-Instruct_embeddings.png}
%         \caption{Embeddings visualization}
%         \label{fig:embeddings}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/Llama-3.2-3B-Instruct_softmax.png}
%         \caption{Softmax visualization}
%         \label{fig:softmax}
%     \end{subfigure}
%     \caption{Representation of embeddings and softmax outputs in Meta Llama 3.2-3B-Instruct model.}
%     \label{fig:embeddings_softmax}
% \end{figure*}


==> figures_latex/softmax.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth]{figures/Llama-3.2-3B-Instruct_softmax.png}
\centering
\caption{Logical level Temporal Bias Analysis using LLama 3.2 3B}
\label{fig:softmax}
\end{figure*}

==> figures_latex/temporal_impact_rq1.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/temporal_impact_semantic.png}
\caption{Temporal impact on semantic integrity}
\label{fig:SemanticTemporalImpact}
\end{figure}

==> old_template/conclusion.tex <==
\section{Conclusion}

==> old_template/discussion.tex <==
\section{Discussion}
....

==> old_template/experiments.tex <==
\section{Experiments}
...

==> old_template/grading.tex <==
\section{Grading}

%Each of the following counts 10 points for your term paper: 
\begin{itemize}
    \item 
\textbf{Writing \& Readability} (30 points): Grammar, Spelling, Formatting (are you using the correct template in Latex?), etc.
%\item \textbf{Readability}: 
Is it easy to follow what you are saying? Is it clear? Is it nicely illustrated with figures and tables? (Your own ones, rather than copy \& paste?)
\item \textbf{Experiment quality} (30 points): how many experiments did you conduct? How thorough are your experiments? How clever are your ideas and your approach? Did you do a nice analysis of limitations and capabilities of your approach? Did you analyze what went wrong and why? 
\item \textbf{Results/Outcome} (30 points): Are your results novel and interesting? Could you beat the state-of-the-art? Did everything fail, so that nothing useful has been obtained? Could you extend previous knowledge? Is there a useful interpretation of your outcomes - e.g., did you shed light on the limitations of certain approaches / techniques (if things didn't go well)?   
\item \textbf{Code repository} (10 points): Is your repository easy to follow and well-structured? Does it contain all necessary aspects (data, code, ...)
\end{itemize}



==> old_template/introduction.tex <==
\section{Introduction}

\paragraph{Structure}
Write your paper as if you were writing a real scientific paper in the Natural Language Processing (NLP) community. Thus, any real NLP paper (e.g., from ACL, NAACL, EMNLP, etc.) may serve as a template for you. 

A typical paper has the following components:
\begin{itemize}
    \item Introduction (1-2 pages): Introduce the topic; illustrate with an easy to understand example; state which problems there are in existing work and how you want to solve them; motivate your paper: what are you actually doing and why (why hasn't it been done until now)
    \item Related work (0.5-1.5 page): Which related papers are there. How does your work differ from them. Which shortcomings does related work have. Typically, you discuss at least 5 different papers and describe each of them by 1-4 sentences
    \item Data (0.5-1.5 pages): Describe the data you use and provide elementary statistics. Data is often neglected, but majorly important. Illustrate your data by giving a couple of real examples. 
    \item Methods (1-3 pages): which approaches are you using? What is your model? Which improvement over existing models do you propose? Use a figure to illustrate your approach.  
    \item Experiments $+$ Results (2-4 pages): Describe: (i) your experimental setup (which hyperparameters, train-dev-test splits); (ii) your baselines and upper bounds (this could also be part of the methods section); (iii) your experimental results (in tables and figures). Finally, (iv) you should also analyze your model: where does it fail? where does it work? Ablations are good to identify important components of your model. 
    \item Discussion (0.5-1 page): What are limitations of your approach? What insights did we gain? What is the wider implication of your findings?
    \item Conclusion (0.25-0.5 page): Summarize and conclude: what did we learn? What could be done in the future to further improve your approach? 
\end{itemize}

\paragraph{Page limits} A typical NLP paper has 8 pages. In this seminar, we aim for 8--10 pages, with an unlimited number of references. Lower and upper limits are strict, i.e., don't write fewer than 8 pages and don't write more than 10 pages. 

\paragraph{Citations} Note that there are two different ways of citing which you should be aware of. The one type is used when the referenced paper is not part of a syntactic component of your sentence; the other is used when it is. The two ways are illustrated here: ``As shown previously, all numbers are equal \citep{Aho:72}. Further, \citet{Chandra:81} show that this holds also for cats.''

\paragraph{Plagiarism} It is important you copy nothing from anywhere. For all that you write, you should \textbf{use your own words}. Also, modifying the sentence structure of the original paper by exchanging individual words counts as plagiarism. Plagiarism will (not only) lead you to failing this course. The best way to avoid plagiarism is not to follow the outline of one particular focus paper that you are discussing but to use your own style and structure. 

\paragraph{Writing style} Try to maintain a \textbf{clear and simple} writing style. In English, it is common to use active voice: ``we conduct the following experiments'' rather than ``the following experiments are conducted''.

\paragraph{Grammar} Having correct English syntax and grammar is important when you write a paper. Bad grammar indicates either: (i) that your education is not so good or that (ii) you do not care --- both of which are bad signals. Be aware of grammar differences to your native language. For example, German speakers have problems with English comma placement (e.g., wrong: ``I believe, that cats are nice''. Right: ``I believe that cats are nice''); in this case, look up correct English comma usage by googling. Another problem for Germans is that in English the passive is not used nearly as often as it is used in German, as mentioned above. People from Asia and Eastern Europe often have problems with articles. Further, Asian natives often have problems with agreement (Wrong: ``They shows''. Right: ``They show''). Look up all these things if they cause you problems.  

Also, take care for things such as quotation marks: ``these are correct'' and ''these are incorrect''.

\paragraph{View-point} In science, it is common to use `we' to refer to yourself (you and your co-authors) when you refer to your own experiments, results, etc. 

\paragraph{Other aspects}
\begin{enumerate}
    \item \textbf{New lines}: When making a new line, just make an empty line in Latex. Do \textbf{not} use two slashes (\textbackslash\textbackslash) followed by ``noindent''. Again, take a real NLP paper as an exemplar.  
    \item \textbf{Talking to the reader}: Do not talk to the reader in the form ``Now, we will show you how to do this properly'' --- this may be common in online tutorials or blogs, but is very very uncommon in scientific papers.
\end{enumerate}

==> old_template/related.tex <==
\section{Related work}

==> old_template/sec1.tex <==
\section{Data}

It is important you use figures, tables (see Table \ref{tab:my_label}), and illustrations. This helps for better understanding of your material.

\begin{table}[!htb]
    \centering
    \begin{tabular}{c|c} \toprule
         Method & Score \\ \midrule
         ABC & 98.4\% \\
         CDE & 92.1\% \\
         \bottomrule
    \end{tabular}
    \caption{Methods and scores; a real caption should be longer and contain all important information to understand the table. Taken from: Paper xyz.}
    \label{tab:my_label}
\end{table}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/Plutchik-wheel-of-emotion.png}
    \caption{Example for figure. Plutchik's wheel of emotions. Use a better and more descriptive caption in a real figure.}
    \label{fig:emotion}
\end{figure}

Make nice looking tables and figures, e.g., using toprule, midrule and bottomrule. 

\textbf{Reference all figures and all tables that you introduce!! E.g., write something like ``Figure \ref{fig:emotion} shows our results and illustrates ...''}

\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/37-barplot-with-number-of-observation.png}
    \caption{Another figure. Make good and telling captions.}
    \label{fig:barplot}
\end{figure*}

==> old_template/sec2.tex <==
\section{Methods}
Use as many sections as you find suitable. 

==> tables/tokenizers.tex <==
\begin{table}[!htp]
\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{SI} & \textbf{TC} & \textbf{PC} & \textbf{PS} \\ \midrule
Baseline      & 1.00 & 4.30 & $\checkmark$ & $\checkmark$ \\
OLMoE         & 0.77 & 5.08 & $\approx$     & $\checkmark$ \\
OLMo          & 0.77 & 5.08 & $\approx$     & $\checkmark$ \\
Davinci-003   & 0.75 & 5.17 & $\times$    & $\checkmark$ \\
Llama 3       & 0.74 & 4.98 & $\times$     & $\checkmark$ \\
GPT-3.5       & 0.74 & 4.98 & $\times$     & $\checkmark$ \\
GPT-4         & 0.74 & 4.98 & $\times$     & $\checkmark$ \\
GPT-4o        & 0.74 & 4.98 & $\times$     & $\checkmark$ \\
Qwen          & 0.42 & 9.30 & $\times$     & $\checkmark$ \\
Cohere        & 0.42 & 9.30 & $\times$     & $\checkmark$ \\
Gemma         & 0.42 & 9.30 & $\times$     & $\checkmark$ \\
DeepSeek      & 0.42 & 9.30 & $\times$     & $\checkmark$ \\
Llama 2       & 0.37 & 10.30 & $\times$    & $\checkmark$ \\
Mistral       & 0.37 & 10.30 & $\times$    & $\checkmark$ \\
Phi 3.5       & 0.37 & 10.30 & $\times$    & $\checkmark$ \\
Llama 1       & 0.37 & 10.30 & $\times$    & $\checkmark$ \\ \bottomrule
\end{tabular}%
}
\caption{Performance comparison of various models on semantic integrity, token count, and preservation of components and separators.}
\label{tab:model_comparison}
\end{table}

